Multi-Item Mechanisms without Item-Independence: Learnability via Robustness

We study the sample complexity of learning revenue-optimal multi-item auctions. We obtain the first set of positive results that go beyond the standard but unrealistic setting of item-independence. In particular, we consider settings where bidders' valuations are drawn from correlated distributions that can be captured by Markov Random Fields or Bayesian Networks -- two of the most prominent graphical models. We establish parametrized sample complexity bounds for learning an up-to-$\varepsilon$ optimal mechanism in both models, which scale polynomially in the size of the model, i.e.~the number of items and bidders, and only exponential in the natural complexity measure of the model, namely either the largest in-degree (for Bayesian Networks) or the size of the largest hyper-edge (for Markov Random Fields). We obtain our learnability results through a novel and modular framework that involves first proving a robustness theorem. We show that, given only ``approximate distributions'' for bidder valuations, we can learn a mechanism whose revenue is nearly optimal simultaneously for all ``true distributions'' that are close to the ones we were given in Prokhorov distance. Thus, to learn a good mechanism, it suffices to learn approximate distributions. When item values are independent, learning in Prokhorov distance is immediate, hence our framework directly implies the main result of Gonczarowski and Weinberg. When item values are sampled from more general graphical models, we combine our robustness theorem with novel sample complexity results for learning Markov Random Fields or Bayesian Networks in Prokhorov distance, which may be of independent interest. Finally, in the single-item case, our robustness result can be strengthened to hold under an even weaker distribution distance, the L\'evy distance.

==> DSIC_robust_multi.tex <==
\section{Dominant Strategy Incentive Compatible Mechanisms}
	 
	 In this section, we show that even in multi-item settings, if every bidder's approximate type distribution $\DD_i$ is within Prokhorov distance $\epsilon$ of her true type distribution $\hDD_i$, given any $\gamma$-DSIC mechanism $M$ for $\DD=\bigtimes_{i=1}^n \DD_i$, we can construct a mechanism $\hM$ in polynomial time such that with probability {almost $1$}, $\hM$ is a {$O(\poly(n,m,\LL,H,\epsilon,\delta))$}-DSIC mechanism for $\hDD=\bigtimes_{i=1}^n \hDD_i$, and its revenue under truthful bidding is at most $O(\poly(n,m,\LL,H,\epsilon,\delta))$ worse than $\rev(M,\DD)$. Formally,
	 
	 \begin{theorem}\label{dsic thm: multi-item p-robustness}
	 	Given $\DD=\bigtimes_{i=1}^n \DD_i$, where $\DD_i $ is a $m$-dimensional distribution for all $i\in[n]$, and a $\gamma$-DSIC mechanism $M$ w.r.t. $\DD$. For any constant $\alpha\in (0,1)$, we can construct a mechanism $\hM$ %\yangnote{in polynomial time given access to the oracle that provides the best bid}
	 	 such that for any possible distribution $\widehat{D}$ close to $D$, that is $\hDD=\bigtimes_{i=1}^n \hDD_i$ satisfying $\norm{\DD_i-\hDD_i}_P\leq \epsilon$ for all $i\in[n]$, with probability at least $1-\alpha$, $\hM$ is a $O(\frac{m\LL\delta+m\LL\gamma}{\alpha})$-DSIC and IR mechanism for $\hDD$, where  $\kappa=O\left( n^2 m \LL H \epsilon+   m \LL\delta\right)$. Moreover, the expected revenue of $\hM$ under truthful bidding is {$$\revT(\hM,\hDD)\geq \rev(M,\DD)-O\left(\frac{n\kappa}{\alpha}\right).$$} 
	 \end{theorem}
	 
	 Let me first sketch our construction, and we break it into three steps. We first sample $\ell$ from $U[0,\delta]^m$ and construct $\round{\DD_i}_{\ell,\delta}$ for every bidder $i$. \begin{itemize}
	
	 	\item Step (i): we construct an $\xi_1$-DSIC mechanism $M_1$ w.r.t. $\bigtimes_{i=1}^n \round{\DD_i}_{\ell,\delta}$, such that $$\revT(M_1, \bigtimes_{i=1}^n \round{\DD_i}_{\ell,\delta})\geq \rev(M,\DD)-O(m \delta)$$ and $\xi_1 = O(m \delta+m\gamma)$.
	 	\item Step (ii): by Lemma~\ref{lem:prokhorov to TV}, we know that w.p. almost $1$, $\norm{\round{\DD_i}_{\ell,\delta}-\round{\hDD_i}_{\ell,\delta}}_{TV}=O(\frac{\epsilon}{\delta})$. We transform $M_1$ into a new mechanism $M_2$ that is $\xi_2$-DSIC w.r.t.  	 $\bigtimes_{i=1}^n \round{\hDD_i}_{\ell,\delta}$. In particular, the construction of $M_2$ does not rely on any information of $\bigtimes_{i=1}^n \round{\hDD_i}_{\ell,\delta}$. Furthermore, $$\revT(M_2, \bigtimes_{i=1}^n \round{\hDD_i}_{\ell,\delta})\geq \revT(M_1, \bigtimes_{i=1}^n \round{\DD_i}_{\ell,\delta})-O(\frac{\epsilon mH}{\delta})$$ and $\xi_2 = O(m\delta+m\gamma)$. 
	 	\item Step (iii): we convert $M_2$ to $\hM$ so that it is well defined for distribution $\hDD$. Again, the conversion does not require any knowledge of $\hDD$. Importantly, $\hM$ will be $O(m\delta+m\gamma)$-DSIC w.r.t. $\hDD$ and $$\revT(\hM, \hDD)\geq \revT(M_1, \bigtimes_{i=1}^n \round{\DD_i}_{\ell,\delta}).$$
	 \end{itemize} 	 
	Next, we prove three Lemmas, one for each step in the proof.

\begin{lemma}\label{dsic lem:original to rounded}
	Given any $\delta>0$, $\ell\in [0,\delta]^m$, and a $\gamma$-DSIC and IR mechanism $M$ w.r.t. $\DD$, we can construct in %\yangnote{polynomial time}
	 a $\xi_1$-DSIC and IR mechanism $M_1$ w.r.t. $\lDD=\bigtimes_{i=1}^n \round{\DD_i}_{\ell,\delta}$, such that $$\revT(M_1, \lDD)= \rev(M,\DD)-nm\LL \delta$$ and $\xi_1 = O(m\LL  \delta + m\LL\gamma)$.
\end{lemma}	 
	\begin{proof}
		We first define $M_1$. Given any bid profile $w\in \supp(\lDD)$, for each bidder $i$  sample $w'_i$ independent from the distribution $\DD_i \mid \bigtimes_{j=1}^m [w_{ij},w_{ij}+\delta)$. Bidder $i$ receives allocation $x_M(w')$ and pays $p_M(w')-m\LL\delta$. Note that  for any $i$ if $w_i$ is drawn from $\round{\DD_i}_{\ell,\delta}$, $w'_{i}$ is drawn from $\DD_i$. If the bidders bid truthfully in $M_1$, the revenue is exactly $\rev(M,\DD)-nm\LL \delta$. Next, we argue that $M_1$ is IR and $\xi_1=O(m\LL\delta)$.
		
		For every bidder $i$ and $w_i\in \supp(\round{\DD_i}_{\ell,\delta})$, for every realization of $w_i'$, its utility for any bid $w'_{-i}$ of all other bidders is \begin{align*}
 	&\E\left [u_i(w_i, M(w_i',w_{-i}'))\right]+m\LL\delta \\
 	\geq & \E \left [u_i(w'_i, M(w_i',w_{-i}'))\right]\\
 	\geq & \E\left [u_i(w'_i, M(x,w_{-i}'))\right] -  m\LL\gamma ~~~~~~~~~~~~~~~~~~~~~~~~~~~~\text{($\forall x\in \supp(\DD_i)$)}\\
 	\geq & \E\left [u_i(w_i, M(x,w_{-i}'))\right] - m\LL\delta -  m\LL\gamma ~~~~~~~~~~~~~~~\text{($\forall x\in \supp(\DD_i)$)}\\
 \end{align*}
		The first inequality is due to the fact that the valuation is $\LL$-Lipschitz. The second inequality is because $M$ is $\gamma$-DSIC w.r.t. $\DD$. The last inequality is again due to the $\LL$-Lipschitzness of the valuation function.
		
		Since $M$ is IR w.r.t. $\DD$, $ \E_{w_{-i}'\sim \DD_{-i}}\left [u_i(w'_i, M(w_i',w_{-i}'))\right]\geq 0$. Hence, $M_1$ is IR w.r.t. $\lDD$. If bidder $i$ reports some  value different from $w_i$, her utility is no more than $$\max_{x\in \supp(\DD_i)} \E\left [u_i(w_i, M(x,w_{-i}'))\right]+m\LL\gamma.$$ Therefore, $M_1$ is $(2m\LL\delta+m\LL\gamma)$-DSIC.
	\end{proof} 
	 
	 By Lemma~\ref{lem:prokhorov to TV}, we know that for any possible true distribution $\hDD$, the rounded distribution $\round{\hDD_i}_{\ell,\delta}$ is close to the rounded approximate distribution $\round{\DD_i}_{\ell,\delta}$ in TV distance for all bidders $i$ with high probability. Intuitively, we should be able to run $M_1$ or a slightly modified version of $M_1$ on distribution $\bigtimes_{i=1}^n \round{\hDD_i}_{\ell,\delta}$ to extract similar revenue. In the next Lemma, we make this intuition formal. Importantly, the way we modify $M_1$ is oblivious to $\hDD$ and $\bigtimes_{i=1}^n \round{\hDD_i}_{\ell,\delta}$.
	 
\notshow{	 \begin{lemma}\label{dsic lem:transformation under TV}
	 	Given any $\delta>0$, $\ell\in [0,\delta]^m$, and a $\eta$-BIC and IR mechanism $M_1$ w.r.t. $\lDD=\bigtimes_{i=1}^n \round{\DD_i}_{\ell,\delta}$, we construct \yangnote{in poly time} a mechanism $M_2$. We show that for any distribution $\FF=\bigtimes_{i=1}^n \FF_i$ that satisfies $\norm{\round{\hDD_i}_{\ell,\delta}-\round{\DD}_{\ell,\delta}}_{TV}$ for all $i\in[n]$, $M_2$ is $\xi_2$-BIC and IR w.r.t. $\hlDD=\bigtimes_{i=1}^n \round{\hDD_i}_{\ell,\delta}$. Moreover, $$\revT(M_2, \hlDD)\geq \revT(M_1, \lDD)-O(\frac{\epsilon mH}{\delta})$$ and $\xi_2 = O(m\delta+\frac{\epsilon mH}{\delta})$. 

	 	
	 	%We show that for any possible true distribution $\hDD$ that satisfies $\norm{\round{\hDD_i}_{\ell,\delta}-\round{\DD}_{\ell,\delta}}_{TV}$ for all $i\in[n]$, $M_2$ is $\xi_2$-BIC and IR w.r.t. $\hlDD=\bigtimes_{i=1}^n \round{\hDD_i}_{\ell,\delta}$. Moreover, $$\revT(M_2, \hlDD)\geq \revT(M_1, \lDD)-O(\frac{\epsilon mH}{\delta})$$ and $\xi_2 = O(m\delta+\frac{\epsilon mH}{\delta})$. 
	 \end{lemma}
	 \begin{proof}
	 	We first construct $M_2$. For any bid profile $w$ in $\supp(\lDD)$, execute $M_1$ on $w$. If bid profile $w\notin \supp(\lDD)$, we execute $M_1$ on bid profile $w'$ where for any bidder $i$ 
  \begin{equation}\label{dsic eq:mapping}
    w_i'=
    \begin{cases}
      w_i, & \text{if}\ w_i\in \supp (\round{\DD_i}_{\ell,\delta})\\
      \argmax_{x\in \supp (\round{\DD_i}_{\ell,\delta})}\E_{b_{-i}\sim \lDD_{-i}}\left[ u_i(w_i,M_1(x,b_{-i}))\right], & \text{otherwise.}
    \end{cases}
  \end{equation}
  
  Clearly, $M_2$ is a well-defined mechanism for any input bid profile, and its construction only depends on $M_1$ and $\lDD$.
  
  Next, we argue that when 	 	%whose bid $w_i$ that is not in $\supp (\round{\DD_i}_{\ell,\delta})$ we change its bid to $$w'_i=\argmax_{x\in \supp (\round{\DD_i}_{\ell,\delta})}\E_{b_{-i}\sim \lDD_{-i}}\left[ u_i(w_i,M_1(x,b_{-i}))\right];$$ if $w_i\in\supp (\round{\DD_i}_{\ell,\delta})$, we choose $w'_i=w_i$.
	 \end{proof}}
	 
	 \begin{lemma}\label{dsic lem:transformation under TV}
	 	Given any distribution $\FF=\bigtimes_{i=1}^n \FF_i$, where each $\FF_i$ is a $m$-dimensional distribution, and a $\eta$-DSIC and IR mechanism $M_1$ w.r.t. $\FF$, we construct %\yangnote{in poly time}
	 	 a mechanism $M_2$. We show that for any distribution $\hFF=\bigtimes_{i=1}^n \hFF_i$ that satisfies $\norm{\hFF_i-\FF_i}_{TV}\leq \nu$ for all $i\in[n]$, $M_2$ is $\eta$-DSIC and IR w.r.t. $\hFF$. Moreover, $$\revT(M_2, \hFF)\geq \revT(M_1, \FF)-O(n^2m\LL H\nu)$$.

	 	
	 	%We show that for any possible true distribution $\hDD$ that satisfies $\norm{\round{\hDD_i}_{\ell,\delta}-\round{\DD}_{\ell,\delta}}_{TV}$ for all $i\in[n]$, $M_2$ is $\xi_2$-BIC and IR w.r.t. $\hlDD=\bigtimes_{i=1}^n \round{\hDD_i}_{\ell,\delta}$. Moreover, $$\revT(M_2, \hlDD)\geq \revT(M_1, \lDD)-O(\frac{\epsilon mH}{\delta})$$ and $\xi_2 = O(m\delta+\frac{\epsilon mH}{\delta})$. 
	 \end{lemma}
	 \begin{proof}
	 	\notshow{We first construct $M_2$. The mechanism has two steps. \begin{enumerate}
	 		\item For any bid profile $w$ in $\supp(\FF)$, execute $M_1$ on bid profile $w'$ where for any bidder $i$ 
  \begin{equation}\label{dsic eq:mapping}
    w_i'=
    \begin{cases}
      w_i, & \text{if}\ w_i\in \supp (\FF_i)\\
      \argmax_{x\in \supp (\FF_i)\cup \perp}\E_{b_{-i}\sim \FF_{-i}}\left[ u_i(w_i,M_1(x,b_{-i}))\right], & \text{otherwise.}
    \end{cases}
  \end{equation}
  \item Pay every bidder an extra amount of $nm\LLH\nu$.
	 	\end{enumerate}   
  Clearly, $M_2$ is a well-defined mechanism for any input bid profile, and its construction only depends on $M_1$ and $\FF$.}
  
  	 	We construct a mechanism $M_2$, and we will show that it is $\eta$-DSIC w.r.t. $\hFF$. For any bid profile $w$ in execute $M_1$ on bid profile $w'$ where for any bidder $i$: 
  \begin{equation}\label{dsic eq:mapping}
    w_i'=
    \begin{cases}
      w_i, & \text{if}\ w_i\in \supp (\FF_i) \ \forall i \in [n] \\
      \argmax_{x\in \supp (\FF_i)\cup \perp}\E\left[ u_i(w_i,M_1(x,w_{-i}))\right] & \text{if only} \ i \in [n] \ \text{is such that} \ w_i \notin \supp  (\FF_i)\\
      \perp
      & \text{otherwise}
    \end{cases}
  \end{equation}


  Next, we argue that when 	$\norm{\hFF_i-\FF_i}_{TV}\leq \nu$ for all $i\in[n]$, $M_2$ is $\eta$-DSIC. Consider any bidder $i$ and any type $w_i\in(-\infty,H]^m$, and any type $x\in\supp(\FF_i)$, we first bound the difference between $\E\left[u_i(w_i,M_1(x,b_{-i}))\right]$ and $\E \left[u_i(w_i,M_2(x,\hb_{-i}))\right]$. Since $\norm{\hFF_i-\FF_i}_{TV}\leq \nu$, we can couple $b_{-i}$ and $\hb_{-i}$ so that $$\Pr[b_{-i}\neq \hb_{-i}]\leq n\nu.$$ Clearly, when $b_{-i}=\hb_{-i}$, $M_1(x,b_{-i})$ has exactly the same allocation and payments as $M_2(x,\hb_{-i})$, and ${ u_i(w_i,M_1(x,b_{-i}))=u_i(w_i,M_2(x,\hb_{-i}))}$. When $b_{-i}\neq \hb_{-i}$, $\left|u_i(w_i,M_1(x,b_{-i}))-u_i(w_i,M_2(x,\hb_{-i}))\right|\leq m\LL H$.
  	Suppose bidder $i$ has type $w_i$, and $w_i'$ is defined as in Equation~\eqref{dsic eq:mapping}, how much more utility can she get by misreporting? If all other bidders report some $b_{-i}$, her utility for reporting her true type is
  	\begin{align}
  	\E\left[u_i(w_i,M_2(w_i,b_{-i}))\right]=&~\E\left[u_i(w_i,M_2(w'_i,b_{-i}))\right]\\ \label{dsic eq:IR}
  	\geq &~ \E\left[u_i(w_i,M_1(w'_i,b_{-i}))\right]\\ 
  	\geq & ~\max_{x\in\supp(\FF_i)}\E\left[u_i(w_i,M_1(x,b_{-i}))\right]-\eta\\
  	\geq & ~\max_{x\in\supp(\FF_i)}\E\left[u_i(w_i,M_2(x,b_{-i}))\right]-\eta\\
  	= & ~ \max_{y\in\mathbb{R}^m}\E\left[u_i(w_i,M_2(y,b_{-i}))\right]- \eta
  \end{align}
	 
	The first equality is because  $M_2(w_i,b{-i})=M_2(w'_i,b_{-i})$. The first inequality is due to true because of the definition of $M_2$. The second inequality is true because $M_1$ is $\eta$-DSIC. The third inequality is again by definition of $M_2$.
	The last equality is because for any $y\in\mathbb{R}^m$ there exists an $x\in\supp(\FF_i)$ such that $M_2(y,b_{-i})=M_1(x,b_{-i})$. Hence, $M_2$ is $\eta$-DSIC. 
	However, $M_2$ may not be IR. Note that for any type $w_i$, the utility for reporting truthfully is also at least $\E\left[u_i(w_i,M_1(w'_i,b_{-i}))\right]$ due to Inequality~\eqref{dsic eq:IR}. If $w_i\in \supp(\FF_i)$,  $$\E\left[u_i(w_i,M_2(w'_i,b_{-i}))\right]= \E\left[u_i(w_i,M_1(w_i,b_{-i}))\right]\geq 0,$$ as $M_1$ is an IR mechanism.
	If $w_i\notin \supp(\FF_i)$, $$ \left[u_i(w_i,M_2(w'_i,b_{-i}))\right]\geq \E\left[u_i(w_i,M_1(\perp,b_{-i}))\right]= 0,$$ so $M_2$ is IR.

	Finally, we show that $\revT(M_2,\hFF)$ is not much less than $\revT(M_1,\FF)$. Let $b\sim \FF$ and $\hb\sim \hFF$. There exists a coupling of $b$ and $\hb$ so that they are different w.p. less than $n\nu$. When $b=\hb$, $M_1(b)=M_2(\hb)$. When $b\neq\hb$, the revenue in $M_1(b)$ is at most $nm\LL H$ more than the revenue in $M'_1(\hb)$. Therefore, $$\revT(M_2,\hFF)\geq \revT(M_1,\FF)-n^2m\LL H \nu.$$
	  	 \end{proof}


In the next Lemma, we make Step (iii) formal.


\begin{lemma}\label{dsic lem:discrete to continuous}
	For any $\delta>0$, $\ell \in [0,\delta]^m$, and distribution $\hDD$, if $M_2$ is a $\xi_2$-DSIC and IR mechanism w.r.t. $\hlDD=\bigtimes_{i=1}^n \round{\hDD_i}_{\ell,\delta}$, we can construct a mechanism $\hM$ oblivious to both $\hDD$ and $\hlDD$, so that $\hM$ is $(\xi_2+2m\LL \delta)$-DSIC and IR w.r.t. $\hDD$. Moreover, $$\revT(\hM,\hDD)= \revT(M_2,\hlDD)-nm\LL\delta.$$
\end{lemma} 

\begin{proof}
	We first construct $\hM$. For any bid profile $w$ in $\supp(\hDD)$, construct $w'=(\rfun(w_1),\ldots,\rfun(w_n))$, and run $M_2$ on $w'$. Bidder $i$ receives allocation $x_{M_2}(w')$ and pays $p_{M_2}(w')-m\LL\delta$. Note that if $w_i\sim \hDD_i$, $w_i'\sim \round{\hDD_i}_{\ell,\delta}$. For any type $b_{-i}$ of all other bidders and $i$'s type is $w_i$, bidder $i$'s utility for bidding truthfully is \begin{align}
 	\E\left[w_i,\hM(w_i,b_{-i})\right]= &~\E\left[w_i,M_2(w'_i,b'_{-i})\right]+m\LL \delta\\
 	\geq &~ \E\left[w'_i,M_2(w'_i,b'_{-i})\right]\label{dsic eq:IR discrete to continuous}\\
 	 	\geq &~ \max_{x\in \supp(\round{\hDD_i}_{\ell,\delta})} \E\left[w'_i,M_2(x,b'_{-i})\right]-\xi_2\\
 	\geq &~ \max_{x\in \supp(\round{\hDD_i}_{\ell,\delta})} \E\left[w_i,M_2(x,b'_{-i})\right]-\xi_2-m\LL \delta\\
 	= & ~ \max_{y\in \supp(\hDD_i)} \E\left[w_i,\hM(y,b_{-i})\right]-\xi_2-2m\LL \delta
 \end{align}
 
 The first and last equalities are due to the definition of $\hM$. The first and the third inequalities are due to the definition of $w_i'$ and the $\LL$-Lipschitzness of the valuation function. The second inequality is because $M_2$ is a $\xi_2$-DSIC mechanism w.r.t. $\hlDD$. By this chain of inequalities, we know that $\hM$ is a $(\xi_2+2m\LL \delta)$-DSIC mechanism w.r.t. $\hDD$. It is not hard to see that $\hM$ is also IR by Inequality~\eqref{dsic eq:IR discrete to continuous}. Finally, if all bidders bid truthfully in $\hM$ when their types are drawn from $\hDD$, its revenue $$\revT(\hM,\hDD)=\revT(M_2,\hlDD)-nm\LL\delta.$$
\end{proof}

Finally, we are ready to prove Theorem~\ref{dsic thm: multi-item p-robustness}.


	 \begin{prevproof}{Theorem}{dsic thm: multi-item p-robustness}
	 	First, sample $\ell$ from $U[0,\delta]^m$, and construct $\round{\DD_i}_{\ell,\delta}$ for all $i\in[n]$. According to Lemma~\ref{dsic lem:original to rounded}, we can construct a mechanism $M_1$ based on $M$ that is $\xi_1 = O(m\LL  \delta + m\LL\gamma)$-DSIC and has revenue $\revT(M_1, \bigtimes_{i=1}^n \round{\DD_i}_{\ell,\delta}) = \rev(M,\DD)-nm\LL\delta$. 
	 	
	 	Next, we argue that $M_1$ can be modified to be a mechanism for distribution $\bigtimes_{i=1}^n \round{\hDD_i}_{\ell,\delta}$ using Lemma~\ref{dsic lem:transformation under TV}. However, to apply Lemma~\ref{dsic lem:transformation under TV}, we will need $\norm{\round{\hDD_i}_{\ell,\delta}-\round{\DD_i}_{\ell,\delta}}_{TV}$ to be small, while we only know $\norm{\DD_i-\hDD_i}_P\leq \epsilon$. This is exactly why we sample $\ell$ randomly from $[0,\delta]^m$. By Lemma~\ref{lem:prokhorov to TV}, \begin{equation}\label{eq:randomized rounding success rate}
	 		\Pr_{\ell\sim U[0,\delta]^m}\left[\norm{\round{\hDD_i}_{\ell,\delta}-\round{\DD_i}_{\ell,\delta}}_{TV}>{n\over \alpha} \left(1+\frac{1}{\delta}\right)\epsilon\right]\leq \alpha/ n
	 	\end{equation} 
	 	for any $\alpha>0$. By the union bound, \begin{equation}\label{dsic eq:good l}
 	\norm{\round{\hDD_i}_{\ell,\delta}-\round{\DD_i}_{\ell,\delta}}_{TV}\leq {n\over \alpha} \left(1+\frac{1}{\delta}\right)\epsilon \text{ for all $i\in[n]$}
 \end{equation}
happens with probability at least $1-1/\alpha$. From now on, we will only consider the case where Equation~\eqref{dsic eq:good l} is true. Choose $\FF_i$ to be $\round{\DD_i}_{\ell,\delta}$, $\hFF_i$ to be $\round{\hDD_i}_{\ell,\delta}$, and $\nu={n\over \alpha} \left(1+\frac{1}{\delta}\right)\epsilon$. We can construct mechanism $M_2$ based on only $M_1$ but not any information about $\hDD$, such that $M_2$ is a $\xi_2=O(\xi_1)$-DSIC and IR mechanism with revenue $\revT(M_2,\bigtimes_{i=1}^n \round{\hDD_i}_{\ell,\delta})\geq \revT(M_1, \bigtimes_{i=1}^n \round{\DD_i}_{\ell,\delta})-O(n^2m\LL H\nu)$.

Finally, Lemma~\ref{dsic lem:discrete to continuous} shows that we can construct $\hM$ using $M_2$, such that $\hM$ is a $(\xi_2+2m\LL\delta)$-DSIC and IR mechanism w.r.t. $\hDD$ with revenue $\revT(\hM,\hDD)=\revT(M_2,\bigtimes_{i=1}^n \round{\hDD_i}_{\ell,\delta})-nm\LL\delta$.

Chain all the inequalities above together. We have that for any constant $\alpha>0$, with probability at least $1-\alpha$, we can construct a mechanism $\hM$ that is $O(\frac{m\LL\delta+m\LL\gamma}{\alpha})$-DSIC, where $$\kappa=O\left( n^2 m \LL H \nu+ m \LL \delta\right)$$ and has revenue $$\revT(\hM,\hDD)\geq\rev(M,\DD)-O\left({n\kappa\over \alpha}\right).$$

We may choose $\delta = n\sqrt{H\epsilon}$ to get 
$$\kappa=O\left( n^2 m \LL H \epsilon+  nm \LL \sqrt{H\epsilon}\right).$$

\end{prevproof}
	 
	 
\begin{theorem}\label{dsic thm:approximation preserving}
	Given $\DD=\bigtimes_{i=1}^n \DD_i$, where $\DD_i $ is a $m$-dimensional distribution for all $i\in[n]$, and a $\gamma$-DSIC mechanism $M$ w.r.t. $\DD$. If $M$ is a $c$-approximation to the optimal $\gamma$-DSIC revenue mechanism for $\DD$, for any constant $\alpha\in (0,1)$, we can construct a mechanism $\hM$ %\yangnote{in polynomial time given access to the optimizer that provides the best bid}
	 such that for any possible true type distribution $\hDD=\bigtimes_{i=1}^n \hDD_i$ satisfying $\norm{\DD_i-\hDD_i}_P\leq \epsilon$ for all $i\in[n]$, with probability at least $1-\alpha$, $\hM$ is a $O(\frac{m\LL\delta+m\LL\gamma}{\alpha})$-DSIC and IR mechanism for $\hDD$. Let $\kappa=O\left( n^2 m \LL H \nu+   m \LL \delta\right)$, where $\nu ={n\over \alpha} \left(1+\frac{1}{\delta}\right)\epsilon$ then the expected revenue of $\hM$ under truthful bidding is {$$\revT(\hM,\hDD)\geq c\cdot\opt(\hDD)-O\left({ n\kappa\over \alpha}\right).$$} 
\end{theorem}
\begin{proof}
	According to Theorem~\ref{dsic thm: multi-item p-robustness}, w.p. $1-\alpha$, we can construct $\hM$ that is $O(\frac{m\LL\delta+m\LL\gamma}{\alpha})$-DSIC and IR w.r.t. $\hDD$, and $\revT(\hM,\hDD)\geq \rev(M,\DD)-O\left(\frac{n\kappa}{\alpha}\right)$. Since $M$ is a $c$-approximation,
	 $\rev(M,\DD)\geq c\cdot \opt_{\gamma}(\DD)$.
	 Similarly, let $M^*$ be a $c$-approximation to the optimal $\gamma$-DSIC revenue mechanism for $\hDD$. Again by Theorem~\ref{dsic thm: multi-item p-robustness}, w.p $1-\alpha$, there exists some mechanism $\widetilde{M}$ that is $O(\frac{m\LL\delta+m\LL\gamma}{\alpha})$-DSIC and IR w.r.t $\DD$ and $\revT(\widetilde{M},\DD) \geq \rev(M^*,\hDD) - O\left(\frac{n\kappa}{\alpha}\right) $ and since $M^*$ is a $c$-approximation, $\rev(M^*,\hDD)\geq c \cdot \opt_{\gamma}(\hDD)$. Chaining the inequalities, the result follows.  
\end{proof}


==> prelim_v2.tex <==
\section{Preliminary}

\begin{definition}[Extension of a Mechanism to All Values]\label{def:mechanism-extension}
 Suppose a mechanism $M$ is defined for all value profiles in $T=\times_{i=1}^n T_i$ where $T_i\subseteq [0,+\infty)$ for $i \in [n]$. Define its extension for all values such that it rounds the bid of each bidder $i$ down to the closest value in $T_i$, and then runs $M$ on the rounded bids. If the bid is smaller than the lowest value in $T_i$, round it to the lowest value of $T_i$, and then run $M$ on the rounded bids. If $M$ assigns the item to bidder $i$, the extended mechanism does not give the item to bidder $i$ and charges her $0$.
\end{definition}
Observe that the extension provides a DSIC and IR mechanism for all values if the original mechanism is DSIC and IR.


\begin{definition}[First-Order Stochastic Dominance]
	We say distribution $B$ \emph{first-order stochastically dominates} $A$ iff $F_B(x)\leq F_A(x)$ for all $x\in \mathbb{R}$. We use $A\preccurlyeq B$ to denote that distribution $B$ first-order stochastically dominates distribution $A$. If $\mathbf{A}=\times_{i=1}^n A_i$ and $\mathbf{B}=\times_{i=1}^n B_i$ are two product distributions, and $A_i\preccurlyeq B_i$ for all $i\in[n]$, we slightly abuse the notation $\preccurlyeq$ to write $\mathbf{A}\preccurlyeq \mathbf{B}$.
\end{definition}

    In the general multiple item setting, $n$ bidders are sold $m$ items, that is outcomes of the auction lie in $X = [0,1]^{n \cdot m}$ such that for any allocation $x \in X$ we have $\sum_{ij}x_{i,j} \leq m$. Allocations of items are then valued by bidders $i \in [n]$ according to a real function $v_i(\cdot): X \rightarrow [0,H]$, which is drawn from some distribution $D_i$. More specifically, we consider valuations where $v_i(\cdot)$ is fully determined by values $(v_{i,1},\ldots,v_{i,m})$ that satisfy the following Lipschitz property. 

\begin{definition}[Lipschitz]
    There exists an absolute constant $L$ such that if $v'_{i,1},\ldots,v'_{i,m}$ is obtained from $v_{i,1},\ldots,v_{i,m}$ by modifying one of the $v'_{i,j}$ by at most an additive $\epsilon$, then $|v_i(x)-v'_i(x)| \leq L\epsilon$ for all $x \in X$.
\end{definition}

This for example includes common settings such as additive and unit demand with Lipschitz constant $L=1$. More generally, $L=1$ holds for additive bidders constrained by being sold at most $k\leq m$ items and even in some settings with complementarities.\\

Mechanisms must be such that bidders have interest to participate and reporting their true value is at least close to their optimal strategy. Formally, given some prices $p=(p_1,\ldots,p_n)$, allocation $x$ and valuation $v$, denote the quasilinear utility of bidder $i\in [n]$ by $u_i(v,x,p) = v_i(x)-p_i(x)$ when the bidders report their true values. 
We say a mechanism $M(v)=(x(v),p(v))$ is individually rational or IR if for all values $v \in [0,H]^{n \cdot m}$ and all bidders $i\in [n]$, $\mathbb{E}[u_i(v_i,M(v))] \geq 0$, where the expectation is taken over the randomness of the mechanism. However, the value reported to $M$ is not necessarily the bidder's true value. Thus we define $M$ to be $\epsilon$-DSIC or Dominant Strategy Incentive Compatible if for all $i\in [n]$, $v\in [0,H]^{n\cdot m}$ and potential misreports $v'_i \in [0,H]^m$ of bidder $i$, $\mathbb{E}[u_i(v_i,M(v))] \geq \mathbb{E}[u_i(v_i,M((v'_i,v_{-i})))] -\epsilon$, where the expectation is taken only over the randomness of $M$. Similarly, define $M$ to be $\epsilon$-BIC or Bayesian Incentive Compatible if the same inequality is satisfied, but this time with the expectation taken over the true values of all bidders but $i$, as well as the randomness of $M$. A mechanism is said to be DSIC or BIC if it is $0$-DSIC or $0$-BIC respectively. 
Moreover, consider some mechanism $\hat{M}$ that is $\epsilon$-BIC for some $\epsilon > 0$ and any distribution $\hat{D}$. We will denote the revenue obtained not by perfectly rational bidders, instead by perfectly truthful ones facing $\hat{M}$, by $\textsc{Rev}_T(\hat{M},\hat{D})$.  Revenue obtained by a BIC mechanism $M$ will simply be $\textsc{Rev}(M,\hat{D})$. Similarly for the revenue of $\epsilon$-DSIC and DSIC mechanisms.\\

Although it is conceivable that permitting mechanisms to be $\epsilon$-BIC allows for greater expected revenue than if they were restricted to be BIC, past results show that in quite general terms, this is not true.

\begin{theorem}[Rubinstein and Weinberg, 2015;
see also Daskalakis and Weinberg, 2012]
Let $\DD$ be any joint distribution over arbitrary valuations, where the valuations of different bidders are independent. The maximum revenue attainable by any IR and $\epsilon$-BIC auction for a given product distribution is at most $2n\sqrt{mLHE}$ greater than the maximum revenue attainable by any IR and BIC auction for that distribution.
\end{theorem}





%\todo{Add the model of valuation}

%\todo{Truthfulness}

%\todo{$\epsilon$-BIC to BIC}
